Adaptive Smolyak Pseudospectral Approximations

Polynomial approximations of computationally intensive models are central to uncertainty quantification. This paper describes an adaptive method for non-intrusive pseudospectral approximation, based on Smolyak's algorithm with generalized sparse grids. We rigorously analyze and extend the non-adaptive method proposed in [6], and compare it to a common alternative approach for using sparse grids to construct polynomial approximations, direct quadrature. Analysis of direct quadrature shows that O(1) errors are an intrinsic property of some configurations of the method, as a consequence of internal aliasing. We provide precise conditions, based on the chosen polynomial basis and quadrature rules, under which this aliasing error occurs. We then establish theoretical results on the accuracy of Smolyak pseudospectral approximation, and show that the Smolyak approximation avoids internal aliasing and makes far more effective use of sparse function evaluations. These results are applicable to broad choices of quadrature rule and generalized sparse grids. Exploiting this flexibility, we introduce a greedy heuristic for adaptive refinement of the pseudospectral approximation. We numerically demonstrate convergence of the algorithm on the Genz test functions, and illustrate the accuracy and efficiency of the adaptive approach on a realistic chemical kinetics problem.

==> ntheoremChapter.tex <==
%%%
%%% This is file `ntheorem.std',
%%% generated with the docstrip utility.
%%%
%%% The original source files were:
%%%
%%% ntheorem.dtx  (with options: `standard')
%%% 
%%% IMPORTANT NOTICE:
%%% 
%%% For the copyright see the source file.
%%% 
%%% Any modified versions of this file must be renamed
%%% with new filenames distinct from ntheorem.std.
%%% 
%%% For distribution of the original source see the terms
%%% for copying and modification in the file ntheorem.dtx.
%%% 
%%% This generated file may be distributed as long as the
%%% original source files, as listed above, are part of the
%%% same distribution. (The sources need not necessarily be
%%% in the same archive or directory.)
%%% This file may be distributed and/or modified under the
%%% conditions of the LaTeX Project Public License, either version 1.2
%%% of this license or (at your option) any later version.
%%% The latest version of this license is in
%%%    http://www.latex-project.org/lppl.txt
%%% and version 1.2 or later is part of all distributions of LaTeX
%%% version 1999/12/01 or later.
%%% \CharacterTable
%%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%%   Dollar        \$     Percent       \%     Ampersand     \&
%%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%%   Asterisk      \*     Plus          \+     Comma         \,
%%%   Minus         \-     Point         \.     Solidus       \/
%%%   Colon         \:     Semicolon     \;     Less than     \<
%%%   Equals        \=     Greater than  \>     Question mark \?
%%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%%   Right brace   \}     Tilde         \~}
%\theoremnumbering{arabic}
%\theoremstyle{plain}
%\theoremsymbol{\ensuremath{_\Box}}
%\theorembodyfont{\itshape}
%\theoremheaderfont{\normalfont\bfseries}
%\theoremseparator{}
%\newtheorem{Theorem}{Theorem}[chapter]
%\newtheorem{theorem}{Theorem}{Theorem}
%\newtheorem{Satz}{Satz}
%\renewtheorem{satz}{Satz}
%\renewtheorem{Proposition}{Proposition}{Theorem}
%\renewtheorem{proposition}{Proposition}{Theorem}
%\renewtheorem{Lemma}{Lemma}
%\renewtheorem{lemma}{Lemma}
%\renewtheorem{Korollar}{Korollar}
%\renewtheorem{korollar}{Korollar}
%\renewtheorem{Corollary}{Corollary}
%\renewtheorem{corollary}{Corollary}
%
%\theorembodyfont{\upshape}
%\renewtheorem{Example}{Example}{Theorem}
%\renewtheorem{example}{Example}{Theorem}
%\renewtheorem{Beispiel}{Beispiel}
%\renewtheorem{beispiel}{Beispiel}
%\renewtheorem{Bemerkung}{Bemerkung}
%\renewtheorem{bemerkung}{Bemerkung}
%\renewtheorem{Anmerkung}{Anmerkung}
%\renewtheorem{anmerkung}{Anmerkung}
%\renewtheorem{Remark}{Remark}
%\renewtheorem{remark}{Remark}
%\renewtheorem{Definition}{Definition}{Theorem}
%\renewtheorem{definition}{Definition}{Theorem}
%
%\theoremstyle{nonumberplain}
%\theoremheaderfont{\scshape}
%\theorembodyfont{\normalfont}
%\theoremsymbol{\ensuremath{_\blacksquare}}
%
%\renewtheorem{Proof}{Proof}{Theorem}
%\renewtheorem{proof}{Proof}{Theorem}
%\renewtheorem{Beweis}{Beweis}
%\renewtheorem{beweis}{Beweis}
%\qedsymbol{\ensuremath{_\blacksquare}}
%\theoremclass{LaTeX}
%
%%%
%%% End of file `ntheorem.std'.

\theoremnumbering{arabic}
\theoremstyle{plain}
\theoremsymbol{\ensuremath{_\Box}}
\theorembodyfont{\itshape}
\theoremheaderfont{\normalfont\bfseries}
\theoremseparator{}
%\newtheorem{Theorem}{Theorem}[section]
%\theorembodyfont{\upshape}
\newtheorem{Example}[Theorem]{Example}
%\newtheorem{Definition}[Theorem]{Definition}
%\newtheorem{Lemma}[Theorem]{Lemma}
%\newtheorem{Remark}[Theorem]{Remark}


\theoremstyle{nonumberplain}
\theoremheaderfont{\scshape}
\theorembodyfont{\normalfont}
\theoremsymbol{\ensuremath{_\blacksquare}}

\newtheorem{Proof}{Proof}
\qedsymbol{\ensuremath{_\blacksquare}}

==> oneDimAndTensor.tex <==
 \section{One Dimensional and Full Tensor Approximations}
\label{sec:approximations}

\subsection{General setting}

\subsection{One-dimensional quadrature}




==> outline.tex <==
\section{Outline}

\begin{easylist}
\ListProperties(Progressive*=3ex)
# Introduction
## Introducing PCEs
### Approximate functions in distribution, useful for a wide variety of problems.
### Intrusive, create systems of equations for coefficients, giving PCEs that tell you the outputs for all inputs, in distribution.
### Non-intrusive has a different purpose, good when you need to sample at smaller spacings than its ``characteristic length''
### MCMC is a good prototype - often calls over and over on points near each other, if $f$ is smooth, this is not necessarily needed
### The idea of a PCE is to approximate a smooth function up front by systematically exploring the likely parameter space, then make it very easy to evaluate.
## Introducing where things went wrong (I need more references for this part)
### Initially, everything was hand tuned and conservative, but when we turn to numeric methods to approximate complex forward models, we need to be more careful
### As we push forward, want to ensure we have the ``right'' strategy
### Forward models are expensive, so we want to make the best possible use of evaluations
### We note that forward models may have low coupling, so quadrature is replaced by sparse quadature, but it's unclear how to synchronize quad/pce
### Some researchers noticed it didn't work as well as interpolation (ie pre Paul's paper)
### Paul showed that significant errors can arise, which are avoided through a smolyak approach (We need to call out his work and contribution in the intro)
## This work - presents a clear and principled way to make PCEs
### We present a Smolyak based approximation scheme for creating PCEs (how do we say it's the same as Paul's, but explained correctly? Say it's a re-interpretation?)
### Smolyak is a principled way to turn 1D algorithms into multivariate algorithms, so we have evidence that it works, and in some cases is optimal or near-optimal
### Allows us to introduce adaptivity derived from DASQ
### Our goal is to present this method, discuss practical considerations, and present enough theory to make our algorithm well founded, although our goal is not especially to provide new proofs of convergence. Maybe we'll adapt some proofs.
### Furthermore, show in detail why the traditional (direct quadrature) strategy doesn't work, and why our method doesn't fall into the same traps
### Finally, make the discussion more practical by discuss practical matters like quadrature, polynomials, growth rules, and convergence

# 1D Polychaos
## Expansion in ortho poly basis
## Converges in distribution for functions in $L_2$.
## show how to compute coeff
## in practice, often substitute integrals for quadrature
## if you use gaussian quadrature, same as interpolation on the same points
## truncation errors in each coeff, discuss their magnitude
## present pce as an operator, maps from function space to function space
## if we can figure it out, show operator error bounds for 1D case

# Extension to Smolyak
## If you're in a tensor product space, Smolyak converts 1D algorithms to sparse tensor algorithms, typically if you have some sort of bounded mixed derivatives, then more efficient than the full tensor algorithms
## Give smolyak formulation
## Useful properties
### Nested gives optimal use
### Nested interpolator gives interpolator, hence equivalence to lagrange interpolation on the same points
### Converges as you get enough terms, clearly state any assumptions needed for this
## This is enough to make this a good idea and usable
## Leaves us with a fair bit of room to alter the 1D rule and thus change the resulting full rule. 
## Explain growth rules and quadrature types.

# Comparison to traditional
## Although in some sense not necessary, we feel it's necessary to be very clear about why the traditional strategy is a bad idea.
## It's tough to be completely general about this, but you don't have general criteria that it converges, as we do for the new method. I don't know how to do an operator bounds proof for all cases.
## Instead, we're going to settle for the Gaussian quadrature case, show two ways it's worse, internal and truncation
## Summary of traditional
### Directly compute coefficients independently via quadrature
### Select a fixed index set for quadrature and a separate index set for your pce, sometimes they're the same
### We don't know of any widespread guidance about how to do this, so it's rather ad hoc
### Adaptive strategies lead us to codify our right strategy is, ad hoc or not
### This gets you into trouble when you try to use the same index set, which intuitively *should* work, the clear candidate for adaptive algorithms
## Contrast methods
### Show which coeff are computed with which quadrature terms
## Internal errors
### Direct sparse quadrature won't work if there is a product of included basis terms that gets you outside the coverage of your quadrature surface
### Smolyak PCE never does that
### Show how even one dimension included will be safe because of telescoping effect
## Truncation Errors
### Truncation errors are the same in the worst case, and have the same source, ie polys outside your quadrature power
### Since Smolyak PCE is more careful than direct quadrature, nearby truncation terms (those that are most likely to be large) have more limited ranges of influence
## All in all, traditional is never better, and often much less accurate than Smolyak PCE. If you fix that, it's going to be much less efficient, since you can't estimate as many pce terms.

# Adaptation
## Back to a method we like.
## The whole point of sparsity is to take advantage of weak coupling, but where is it? Often don't know in advance.
## DASQ provides a perfect model, add terms to refine terms that alter your estimate the most, it's trivial to adjust to another Smolyak algorithm
## The combined method has one place for adaptivity, it's much clearer than the direct quad strategy.
## Simple, probably effective, but heuristic.
## Can't help you for pathological cases with arbitrary blocks of zeros and non-zeros.
## We know coeff will eventually decay exponentially, just need to initialize with enough terms for this to kick in (rightfully hard to determine). Furthermore, extra terms should induce errors in useful places to suggest where to go. Although, I'm not going to swear to that.
## Biggest question is which norm-ish value to use. An upper bound on the variance is a decent way to go.
## We need to settle the question about which terms are expandable - I differ from DASQ. Not sure if I'm right, he's right, or there's no clear reason for either one. 
## Should you consider how much work the terms are? Probably. Haven't done that yet.

# Other practical matters - quadrature selection
## We know nestedness is not necessary, but is really nice. Gauss patterson is nice, guaranteed poly order, but there's only a few levels.
## Although not perfect, clenshaw curtis is good, transplanted is awesome. Possibly more stable than Gauss for truncated terms (some evidence in the paper for this). Hard to prove some of the previous things for, but maybe a good idea anyway.
## We have to handle different measures - then what? Since measures are often analytic, transplanted clenshaw curtis may still work? Maybe you need higher order for each rule?
## Linear growth should always skip by 2 to avoid even/oddness.
## Maybe we could construct patterson for other measures? Possible but super annoying because they're almost unstable to generate? (yay mathemetica?)
## Exp growth gauss will work, pretty simple, even though it's not optimal

# Experiments
## Don't bother to compare to traditional, will have shown previously just how bad it does, is no longer a fair reference with theory showing how bad it is
## Instead, compare against different attempts to use isotropic shapes
## Hopefully, on moderately sized examples, try to show that against the ``true'' solution, adaptation can pick the right terms, and compute them almost right. Compare the different growth strategies we want to recommend. Possibly L2 convergence or capturing the variance correctly is a good measure
## Make sure we do both Legendre and Hermite examples.

# Conclusions
## Smolyak PCE is principled and efficient, so its definitely the way to go. 
## Still allows a bit of freedom in index sets and quadature, which we can exploit to make it go faster.
## In lieu of rigorous theory about the exact limited space our function lives in, just use adaptation to figure it out
## Make suggestions about the right quadrature rules/sequences to use, although this part isn't definite

\end{easylist}






==> problemDefs.tex <==
% hilbert space L2(X, \mu) of square integrable functions on X with weighted inner product [define]

% tensor product of hilbert spaces: functions on X_1 \times X_2

% what about operators? Operators (e.g., integral, projection) act on a tensor product space. Can define the operators themselves as tensor products


\section{One Dimensional and Tensor Problems}
\label{sec:problems}

\subsection{General setting}


\subsection{One-dimensional integration}


\subsection{Multi-dimensional integration}

One-dimensional integration extends easily to higher-dimensional integrals over product domains with separable weight functions. Let $X^{(1)}, \ldots, X^{(d)}$ be a collection of intervals on the real line, as in the one dimensional case. Then let 
%
\begin{equation}
\mathbf{X} := X^{(1)} \times \cdots \times X^{(d)} \subseteq \mathbb{R}^d
\end{equation}
%
be the domain of integration, defined by the Cartesian product of one-dimensional intervals. Consider a real-valued function defined on this product space, $f:\mathbf{X} \to \mathbb{R}$. Then the multi-dimensional integral is given by the tensor product of one-dimensional integral operators:
\begin{eqnarray}
\label{eq:multi-int}
\mathcal{I}^{(\mathbf{d})}(f) & = & \mathcal{I}^{(1)} \otimes \cdots \otimes \mathcal{I}^{(d)} (f) \nonumber \\
&= &\int_{X^{(1)}} \ldots \int_{X^{(d)}} w^{(1)}(x^{(1)}) \ldots w^{(d)}(x^{(d)}) f(x^{(1)}, \ldots, x^{(d)}) \, dx^{(d)} \ldots dx^{(1)} \\
 &=& \int_\mathbf{X} w(\mathbf{x})f(\mathbf{x}) \, d \mathbf{x}, \nonumber \\
\mbox{where } w(\mathbf{x}) &:=& \prod_{i=1}^d w^{(i)}({x}^{(i)}) . \nonumber
\end{eqnarray}
%
% These integrals have a simple structure: the weight function is separable and the domain is a rectangle.




% \begin{align}
% \mathcal{P}^{(\mathbf{d})} &= \mathcal{P}^{(1)} \otimes \cdots \otimes \mathcal{P}^{(d)}
% \end{align}


% Stye note: if $\mathbf{n}$ is vector, its components $n_i$ should not be boldface
